Learning to Drive from a World Model

Most self-driving systems rely on hand-coded perception outputs and engineered driving rules. Learning directly from human driving data with an end-to-end method can allow for a training architecture that is simpler and scales well with compute and data. In this work, we propose an end-to-end training architecture that uses real driving data to train a driving policy in an on-policy simulator. We show two different methods of simulation, one with reprojective simulation and one with a learned world model. We show that both methods can be used to train a policy that learns driving behavior without any hand-coded driving rules. We evaluate the performance of these policies in a closed-loop simulation and when deployed in a real-world advanced driver-assistance system.

==> training_config.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lc}
    \toprule
    Optimizer                   & AdamW        \\
    Optimizer betas             & (0.9, 0.95)  \\
    Learning rate               & 1e-4         \\
    Steps                       & 409,600      \\
    Linear warmup               & 10\% steps   \\
    Linear decay                & 90\% steps   \\
    Weight decay                & 1e-2         \\
    Batch size                  & 512          \\
    Clip grad norm              & 1.0          \\
    Number of parameters        & 500M and 1B    \\
    Number of training minutes  & 500k and 2.5M    \\
    \bottomrule
    \end{tabular}
    \caption{Training hyperparameters.}
    \vspace{-0.05in}
    \label{tab:training_config}
\end{table}

==> world_model_results_test_lpips_obs_act_forced.tex <==
% https://reporter.comma.life/experiment/155a130c-ed4a-4a73-8bbf-3a5ad639b712
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{results_test_lpips_obs_act_forced.pdf}
    \caption{Observation and action teacher-forced next frame prediction LPIPS. Note that the prediction improves as the model gets closer to the future anchoring.}
    \label{fig:worldmodel_simulation_results_test_lpips_obs_act_forced}
    \vspace{-0.05in}
\end{figure}

==> world_model_simulation_deviation_future_vs_no_future.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.35\textwidth]{deviation_RIGHT_future_vs_no_future.png}
    \caption{We force a lateral deviation of $0.5$m using Reprojective Simulation. Blue: trajectory from a Future Anchored Plan Model. Red: trajectory from a Non-Future Anchored Plan Model.}
    \vspace{-0.05in}
    \label{fig:worldmodel_simulation_deviation_future_vs_no_future}
\end{figure}
